On the support recovery of marginal regression

Leading methods for support recovery in high-dimensional regression, such as Lasso, have been well-studied and their limitations in the context of correlated design have been characterized with precise incoherence conditions. In this work, we present a similar treatment of selection consistency for marginal regression (MR), a computationally efficient family of methods with connections to decision trees. Selection based on marginal regression is also referred to as covariate screening or independence screening and is a popular approach in applied work, especially in ultra high-dimensional settings. We identify the underlying factors---which we denote as \emph{MR incoherence}---affecting MR's support recovery performance. Our near complete characterization provides a much more nuanced and optimistic view of MR in comparison to previous works. To ground our results, we provide a broad taxonomy of results for leading feature selection methods, relating the behavior of Lasso, OMP, SIS, and MR. We also lay the foundation for interesting generalizations of our analysis, e.g., to non-linear feature selection methods and to more general regression frameworks such as a general additive models.

==> proofs.tex <==
\section{Proof of Theorem~\ref{thm:MR:main:res}}
\label{sec:proofs}
%\subsection{Theorem~\ref{thm:MR:main:res}}
Under model~\eqref{eq:lin:model:pop} $\cov(X,Y) = \ex X(X^T \beta + \eps) = \Sigma \beta$, that is $\cov(X_j,Y) = \ip{\Sigma_{*j},\beta}$ where $\Sigma_{*j}$ is the $j$th column of $\Sigma$.
If follows that MR achieves exact support recovery over $\Gamma_S$ with slack $\delta$ in the sense of~\eqref{eq:pop:supp:recovery:slack:def} if and only if %\aaa{Is this true the way we defined it}
%\begin{align}
%\min_{j\, \in\, S} |\ip{\Sigma_{*j},\beta}| > \delta + \max_{k \, \in\, S^c} |\ip{\Sigma_{*k},\beta}|,\quad \forall \beta \in \Gamma_S 
%\end{align}
%or equivalently
\begin{align}\label{eq:mr:recovery:cond:1}
|\ip{\Sigma_{*k},\beta}| + \delta < |\ip{\Sigma_{*j},\beta}|,\quad \forall \beta \in \Gamma_S,\; j \in S,\; k \in S^c.
\end{align}
%This is an extended version of the Faithfulness condition in~\cite{Genovese2012}, restated for all $\beta \in \Gamma_S$.
%\begin{lem} Let $\phi_0,\phi_1 \in \reals^p$ and $\Gamma \subset \reals^p$. The following two statements are equivalent: 
%	\begin{enumerate}[label=(\alph*)]
%		\item $|\ip{\phi_1, \beta}| > \delta + |\ip{\phi_0, \beta}|$ for all $\beta\in \Gamma$.
%		\item $|\ip{\phi_1 + \lambda \phi_0, \beta}| > \delta$ for all $\beta\in \Gamma$ and all $\lambda \in [-1,+1]$.
%	\end{enumerate}
% %if and only if 
%\end{lem}
%
%\begin{proof}
%Fix $\beta\in \Gamma$ for the entire proof. 
%
%$(b)\implies (a)$. Due to the identity $\min \{|a+b|,\; |a-b|\} = |\,|a| - |b|\,|$, we have
%$$
%\min \{ |\ip{\phi_1 + \lambda \phi_0, \beta}|,\; |\ip{\phi_1 - \lambda \phi_0, \beta}| \} = |\,|\ip{\phi_1, \beta}| - |\lambda|\cdot |\ip{\phi_0, \beta}|\,| 
%$$ 
%Define $g(\lambda) = |\ip{\phi_1, \beta}| - |\lambda|\cdot |\ip{\phi_0, \beta}|$. From $(b)$ and the identity above, we know
%$$
%|g(\lambda)| > \delta,\quad \forall \lambda \in [-1,1]
%$$
%Therefore $g(\lambda)$ never gets zero. Since it is a continuous function, it never changes sign either. Because $g(\lambda) = |\ip{\phi_1, \beta}| \geq 0$, it must be positive for all $\lambda \in [-1, 1]$, and in particular for $\lambda=1$.
%
%$(a) \implies (b)$. This direction is easier. Take any $\lambda \in [-1, 1]$,
%\begin{align*}
%\delta &< |\ip{\phi_1, \beta}| - |\ip{\phi_0, \beta}| \\
%&\leq |\ip{\phi_1, \beta}| - |\lambda|\cdot |\ip{\phi_0,  \beta}| \\
%&\leq |\ip{\phi_1, \beta} + \lambda \ip{\phi_0,  \beta}| \\
%&= |\ip{\phi_1 + \lambda \phi_0, \beta}|
%\end{align*}
%
%\end{proof}

\begin{lem}\label{lem:a:b:lambda}
	For any $a,b \in \reals$ and $\delta > 0$, we have $|a| - |b| > \delta  \iff  |a-\lambda b| > \delta,\; \forall \lambda \in [-1,1].$

\end{lem}

Using Lemma~\ref{lem:a:b:lambda}, condition~\eqref{eq:mr:recovery:cond:1} is equivalent to $|\ip{\Sigma_{*j}+\lambda \Sigma_{*k}, \beta}| > \delta$ for all $\beta\in \Gamma_S,\; j\in S, \; k\in S^c$ and $\lambda\in [-1,1]$. For a set $\Gamma \subset \reals^p$, we define its \emph{absolute dual} with slack $\delta$ to be 
\begin{align}\label{eq:abs:dual:def}
\Gamma^\dagger= \big\{ \phi \in \reals^p :\; |\ip{\phi, \beta}| > \delta,\; \forall \beta \in \Gamma \big\}.
\end{align}
Thus, exact support recovery by MR over $\Gamma_S$ with slack $\delta$ is equivalent to
\begin{align}\label{eq:mr:recovery:cond:2}
	\Sigma_{*j}+\lambda \Sigma_{*k} \in \Gamma_S^\dagger, \quad \text{for all}\; (j,k) \in S\times S^c, \; \text{and}\;\lambda \in [-1,1].
\end{align}
%
%\begin{lem}
%The absolute dual of $\Gamma_S$ given in~\eqref{eq:Gamma:S:def} satisfies
%\begin{align*}
%	\Gamma_S^\dagger \,\supseteq\, \Big\{\phi \in \reals^p \,  : \,\, \|\phi_S\|_\infty > \frac{\delta}{\rho (1+R)}+ \frac{R}{1+R} \|\phi_S\|_1 \Big\} =:\Gamma_S'.
%\end{align*}
%\end{lem}
The following technical lemma, proved in Appendix~\ref{sec:rem:proof}, characterizes the absolute dual of the parameters space  $\Gamma_S$:
\begin{lem}\label{lem:Gamma:S:identify}
	The absolute dual of $\Gamma_S$ given in~\eqref{eq:Gamma:S:def} can be written as $\Gamma_S^\dagger = \Gamma_S' \cup \Omega_S$ where 
	\begin{align*}
	\Gamma_S' &:= \Big\{\phi \in \reals^p \,  : \,\, \|\phi_S\|_\infty > \frac{\delta}{\rho (1+R)}+ \frac{R}{1+R} \|\phi_S\|_1 \Big\} , \\
	\Omega_S \subseteq \Gamma_S'' &:= \Big\{\phi \in \reals^p \,  : \,\, \|\phi_S\|_\infty < -\frac{\delta}{\rho (1+R)}+ \frac{1}{1+R} \|\phi_S\|_1 \Big\}.
	\end{align*}
%	and
%	\begin{align*}
%	\Gamma_S^\dagger\backslash \Gamma_S' \,\subseteq\, \Big\{\phi \in \reals^p \,  : \,\, \|\phi_S\|_\infty < -\frac{\delta}{\rho (1+R)}+ \frac{1}{1+R} \|\phi_S\|_1 \Big\} =:.
%	\end{align*}
\end{lem}



%\begin{proof}
%Take any $\beta \in \Gamma_S$ and $\phi \in \Gamma_S'$.
%%assume $\phi\in \reals^p$ has this property:
%%$$
%%\|\phi_S\|_\infty > \frac{\delta}{\rho (1+R)}+ \frac{R}{1+R} \|\phi_S\|_1
%%$$
%Let $j \in \text{argmax}_{j'\in S}\; |\phi_{j'}|$. Then,
%\begin{align*}
%|\ip{\phi, \beta}| &= |\ip{\phi_S, \beta_S}| \\
%&\geq |\phi_{j}|\; |\beta_{j}| - \big| \sum_{j'\in S\backslash \{j\}} \phi_{j'}\;\beta_{j'}\big| \\
%&\geq |\phi_{j}|\; |\beta_{j}| - \sum_{j'\in S\backslash \{j\}} |\phi_{j'}|\; |\beta_{j'}| \\
%&\geq \|\phi_S\|_\infty \; \min_{j\in S} |\beta_j| - (\|\phi_S\|_1 - \|\phi_S\|_\infty)\; \|\beta_S \|_\infty \\
%&\overset{(i)}{\geq} \|\phi_S\|_\infty \; \min_{j\in S} |\beta_j| - R\;(\|\phi_S\|_1 - \|\phi_S\|_\infty)\; \min_{j\in S} |\beta_j| \\
%&\overset{(ii)}{>} \frac{\delta}{\rho} \; \min_{j\in S} |\beta_j|  \\
%&\overset{(iii)}{\geq} \delta,
%\end{align*}
%where (i) and (iii) are implied by $\beta \in \Gamma_S$ and (ii) by $\phi \in \Gamma_S'$.
%\end{proof}
%

\begin{proof}[Theorem~\ref{thm:MR:main:res}(a)]
	Let $\delta' = \delta/ \rho$. By Lemma~\ref{lem:Gamma:S:identify}, $\Gamma'_S \subset \Gamma_S^\dagger$. Hence, replacing $\Gamma_S^\dagger$ in~\eqref{eq:mr:recovery:cond:2} with $\Gamma_S'$ we get the following sufficient condition for recovery:
	\begin{align}\label{eq:temp:cond:0} 
	\frac{R}{1+R} \|\Sigma_{Sj}+\lambda \Sigma_{Sk} \|_1 +  \frac{\delta'}{1+R} < \infnorm{\Sigma_{Sj}+\lambda \Sigma_{Sk}},
	\quad \forall j\in S, \;k\in S^c,\; \lambda\in [-1,1].
	\end{align}
	%We will shortly show:
	We have (see Appendix~\ref{sec:rem:proof} for the proof):
	\begin{lem}\label{lem:infnorm:equality}
		Condition~\eqref{eq:temp:cond:0} implies $\| \Sigma_{Sj}+\lambda \Sigma_{Sk} \|_\infty =  \Sigma_{jj}+\lambda \Sigma_{jk}$ for all $\lambda\in [-1,1]$.
	\end{lem} 
	%\begin{align}\label{eq:infnorm:equal:top:elm}
	%	\| \Sigma_{Sj}+\lambda \Sigma_{Sk} \|_\infty =  \Sigma_{jj}+\lambda \Sigma_{jk}
	%\end{align}
	Therefore, \eqref{eq:temp:cond:0} implies
	\begin{align}\label{eq:temp:cond:1}
	 \frac{R}{1+R} \|\Sigma_{Sj}+\lambda \Sigma_{Sk} \|_1 + \frac{\delta'}{ 1+R} < \Sigma_{jj}+\lambda \Sigma_{jk},\quad \forall j\in S, \,k\in S^c, \,\lambda\in [-1,1].
	\end{align}
	In the other direction, \eqref{eq:temp:cond:1} clearly implies~\eqref{eq:temp:cond:0} noting that $\| \Sigma_{Sj}+\lambda \Sigma_{Sk} \|_\infty  \ge $ $\Sigma_{jj}+\lambda \Sigma_{jk} \ge 0$ for all $|\lambda|\le1$, since by assumption $\Sigma_{jj} = 1$ hence $|\Sigma_{jk}| \le 1$. Since the RHS of~\eqref{eq:temp:cond:1} is convex in $\lambda$ and the LHS is linear, \eqref{eq:temp:cond:1} holds if and only if it holds at the two endpoints $\lambda = -1,1$ which gives~\eqref{eq:MR:incoh} as desired.
\end{proof}


\begin{proof}[Theorem~\ref{thm:MR:main:res}(b), case $R \ge 2$]
	%In the remainder of the proof, 
	Assume $\rho=1$ without loss of generality. We also write $\Gamma_{S,R} = \Gamma_S$ to emphasize the dependence on $R$.
	For any $\phi\in \reals^p$, let us define 
	\begin{align*}
	\alpha_R(\phi) = \min_{\beta \,\in\, \Gamma_{S,R}} |\ip{\phi, \beta}|
	\end{align*}
	By definition, $\phi$ belongs to $\Gamma_{S,R}^\dagger$
	if and only if $\alpha_R(\phi)> \delta$.  An interesting case is when $R=1$, in which case we use the notation $\alpha(\phi)$ instead of $\alpha_1(\phi)$. The minimization in the case of $R=1$ is over $\Gamma_{S,1}$, which consists of vectors with $\pm \rho$ coordinates on the support. For any $\beta \in \Gamma_{S,1}$, it is easy to see that
	\begin{align}\label{eq:inner:prod:identity}
	\ip{\phi, \beta} = \sum_{j\in S_1} |\phi_j| - \sum_{j \in S_0} |\phi_j| 
	\end{align}
	%\aaa{$\rho$ is missing from subsequent discussion. We can assume $\rho = 1$ without loss of generality. }
	where $S_1 = \{j\in S \; : \; \sign(\beta_j) = \sign(\phi_j)\}$ and $S_0 = S\backslash S_1$. The relation works both ways, i.e., for any partition of $S$ into $S_1$ and $S_0$, there exists a $\beta\in \Gamma_{S,1}$ that \eqref{eq:inner:prod:identity} holds. %\aaa{Overload of notation regarding $S_0,S_1$ with that in~\eqref{eq:min:inner:prod:identity}, changed the one in~\eqref{eq:min:inner:prod:identity}.}
	
	Let $\{S_0(\phi), S_1(\phi)\}$ be any partition that achieves the minimum for $\phi$ %\aaa{not unique in general?}
	such that $S_1(\phi)$ corresponds to the larger of the two sums, that is
	% An interesting partition is the one that achieves the minimum:
	\begin{align}\label{eq:min:inner:prod:identity}
	\alpha(\phi) = \sum_{j \,\in\, S_1(\phi)} |\phi_j| - \sum_{j \,\in\, S_0(\phi)} |\phi_j| \ge 0.
	\end{align}
	Note that whenever $\phi \neq 0$, we have $|S_1(\phi)| \ge 1$ with $|\phi_j| > 0$ for at least some $j \in S_1(\phi)$. %\aaa{Please check, might be wrong. In general we have to the address the case where $S_1$ is empty which seems not possible unless $\phi = 0$. }
	We  adopt the convention of putting the indices of the zero coordinates of $\phi$ in $S_0(\phi)$. Thus, for $\phi \neq 0$, we have $\min_{j \in S_1(\phi)} |\phi_j| > 0 $. 
	As the following lemma states, $\alpha(\phi)$ can be used to approximate $\alpha_R(\phi)$.
	
	\begin{lem}\label{lem:alpha:R:bound}
		If $\phi\in \Gamma_{S,R}^\dagger \setminus \Gamma_{S,R}'$, then \;$\alpha_R(\phi) \leq \max \big\{0, (2-R)\, \alpha(\phi) \big\}$.
	\end{lem}
	As a consequence, $\Gamma_S^\dagger = \Gamma_S'$ whenever $R\geq 2$, completing the proof of part~(b).
\end{proof}

\begin{proof}[Theorem~\ref{thm:MR:main:res}(b), case $\Sigma_{SS} = I$]
	Fix $k\in S^c$. Let $j^*\in \text{argmin}_{j'\in S} |\Sigma_{j'k}|$ and choose $\beta\in \Gamma_{S,\rho,R}$ such that
	\begin{align*}
	\beta_{j^*} = \sign(\Sigma_{j^*k})\,\rho, \quad %\text{and} \quad 
	\beta_{j'}=\sign(\Sigma_{j'k})\,R\rho, \; \;\forall j'\in S\backslash \{j^*\}.
	\end{align*}
	Selection consistency implies that
	\begin{align*}
	R\rho\; \|\Sigma_{Sk}\|_1  - (R\rho - \rho)\; |\Sigma_{Sk}|_{\min} + \delta = |\ip{\Sigma_{Sk}, \beta}| +\delta < |\ip{\Sigma_{Sj^*}, \beta}| =  \rho
	\end{align*}
	using assumption $\Sigma_{SS}=I$ in the last equality. Dividing by $\rho$ and rearraging proves~\eqref{eq:mr:incoh:SigSS:I} which is equivalent to~\eqref{eq:MR:incoh:2}, due to Lemma~\ref{lem:mr:incoh:SigSS:I}.
\end{proof}



%Now, considering the convexity of RHS and linearity of LHS, we conclude another equivalent form

